Vlaser: Vision-Language-Action Model with Synergistic Embodied Reasoning

While significant research has focused on developing embodied reasoning capabilities using Vision-Language Models (VLMs) or integrating advanced VLMs into Vision-Language-Action (VLA) models for end-to-end robot control, few studies directly address the critical gap between upstream VLM-based reasoning and downstream VLA policy learning. In this work, we take an initial step toward bridging embodied reasoning with VLA policy learning by introducing Vlaser - a Vision-Language-Action Model with synergistic embodied reasoning capability, which is a foundational vision-language model designed to integrate high-level reasoning with low-level control for embodied agents. Built upon the high-quality Vlaser-6M dataset, Vlaser achieves state-of-the-art performance across a range of embodied reasoning benchmarks - including spatial reasoning, embodied grounding, embodied QA, and task planning. Furthermore, we systematically examine how different VLM initializations affect supervised VLA fine-tuning, offering novel insights into mitigating the domain shift between internet-scale pre-training data and embodied-specific policy learning data. Based on these insights, our approach achieves state-of-the-art results on the WidowX benchmark and competitive performance on the Google Robot benchmark.

==> Tables/rebuttal_compare_qwen.tex <==
\begin{table}[ht!]
% \scriptsize
% \vspace{-2mm}
\centering
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\linewidth}{!}{
\begin{tabular}{lcccc|cccc|}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}}  & \multicolumn{4}{c|}{Embodied Grounding}                    & \multicolumn{4}{c|}{Planning \& Simulation}                \\
\multicolumn{1}{c}{}                 & \textbf{Where2place} & \textbf{Pointarena}   & \textbf{Paco-Lavis}   & \textbf{Pixmo-Points} & \textbf{Ego-Plan2}       & \textbf{VLABench} & \textbf{EB-ALFRED} & \textbf{EB-Habitat}                      \\
\midrule

Qwen2.5VL-3B       &   69.0   &   56.2 &  77.6 &   36.9  & 40.5 &  31.2 &  43.7 & 31.1                                          \\

Qwen2.5VL-7B       &   65.2    &   59.7 &  73.1 &  37.8 & 55.2   & 44.4 &  51.2 & 38.9                \\


\bottomrule
\end{tabular}
}

\label{tab:mllm_benchmark}
\vspace{-1em}
\end{table}

==> Tables/rebuttal_embodied_reasoning_data.tex <==
\begin{table}[ht!]
% \scriptsize
% \vspace{-2mm}
\centering
\setlength\tabcolsep{1.5pt}
\renewcommand{\arraystretch}{1.15}
% \caption{\textbf{Comparison with existing close-sourced, open-sourced and embodied-related VLMs on 12 general embodied reasoning benchmarks, spanning from embodied QA, planning, embodied grounding to spatial intelligence and close-loop simulation evaluation.}  Avg denotes the  normalized average performance of all the benchmarks. The best, second best and third best score among all the baselines are colored in red, orange and yellow.}
\resizebox{\linewidth}{!}{
\begin{tabular}{lc|ccc|cc|ccc|c}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{Model}} & QA  & \multicolumn{3}{c|}{Embodied Grounding}                   & \multicolumn{2}{c|}{Spatial Intelligence} & \multicolumn{3}{c|}{Planning \& Simulation}               & \multicolumn{1}{c}{\multirow{2}{*}{Avg}} \\
\multicolumn{1}{c}{}                       & \textbf{ERQA}               & \textbf{Where2place} & \textbf{Pointarena}   & \textbf{Paco-Lavis}    & \textbf{VSIBench}  & \textbf{RefSpatial}  & \textbf{Ego-Plan2}       & \textbf{VLABench} & \textbf{EB-ALFRED}  & \multicolumn{1}{c}{}                     \\
\midrule


InternVL3-2B  &  31.5 &	5.2 &	7.1 &	15.4 &	31.5 &	1.8 	& 30.9 &	19.4 &	1.3 &	16.0                                                                 \\
+ 1.8M Embodied Grounding Data  & 31.5	& 79.2	& 60.3	& 80.1	& 27.9 &	20.2	& 15.4	& 16.2	& 0.2	& 36.8                                                              \\
+  1.2M General QA Data      &  36.8	& 78.8 &	61.1	& 74.2	& 28.8	& 23.5	& 22.3	& 20.1	& 20.1	& 40.6                                  \\
+ 600k Spatial Reasoning Data    &  36.2 &	75.1 &	55.5 &	74.4 &	59.8 &	42.7 &	21.8 &	18.7 &	21.3 &	45.1                                     \\
+ 400k Planning Data  & 35.8 &	74.0 &	57.8 &	72.5 &	57.5 	& 43.0 &	38.3 &	23.1 &	42.3 &	49.4                                                                     \\                        
% \todo{janus?} \\
% \todo{other sota 2B MLLM (see opencompass)} \\


\bottomrule
\end{tabular}
}
% \caption{\textbf{Comparison with existing MLLMs and VLAs on general MLLM benchmarks.} ``\#A-Param'' denotes the number of activated parameters. For MME, we sum the perception and cognition scores.   Avg denotes the  normalized average performance of MLLM benchmarks and VQA benchmarks. The highest score among open-source MLLMs and VLAs are colored in bold.}

\label{tab:mllm_benchmark}
\vspace{-1em}
\end{table}
